Explicit Feature Interaction-aware Graph Neural Networks

Graph neural networks (GNNs) are powerful tools for handling graph-structured data. However, their design often limits them to learning only higher-order feature interactions, leaving low-order feature interactions overlooked. To address this problem, we introduce a novel GNN method called explicit feature interaction-aware graph neural network (EFI-GNN). Unlike conventional GNNs, EFI-GNN is a multilayer linear network designed to model arbitrary-order feature interactions explicitly within graphs. To validate the efficacy of EFI-GNN, we conduct experiments using various datasets. The experimental results demonstrate that EFI-GNN has competitive performance with existing GNNs, and when a GNN is jointly trained with EFI-GNN, predictive performance sees an improvement. Furthermore, the predictions made by EFI-GNN are interpretable, owing to its linear construction. The source code of EFI-GNN is available at https://github.com/gim4855744/EFI-GNN

==> algorithms/gcn_cross_train.tex <==
\begin{algorithm}[t!]

    \caption{Forward Propagation of EFI-GNN}
    
    \begin{flushleft}
        \textbf{Input}:\\
            \hspace{4pt} normalized adjacency matrix $\hat{\textbf{A}}$\\
            \hspace{4pt} raw feature matrix $\textbf{X}^{(0)}$\\
            \hspace{4pt} target labels $\textbf{Y}$\\
            \hspace{4pt} number of layers $L$ \\
        \textbf{Parameter}:\\
            \hspace{4pt} trainable weights $\textbf{W}^{(1)}$, $\textbf{W}^{(2)}$, ..., $\textbf{W}^{(L)}$, $\textbf{W}^{(\text{out})}$
    \end{flushleft}
    
    \begin{algorithmic}[1] %[1] enables line numbers
    
        \State $\textbf{X}^{(1)} = \text{matmul}(\textbf{X}^{(0)}, \textbf{W}^{(1)})$ \Comment{sum of 1st-order features}
        \vspace{0.3cm}

        \For{$i=1$ to $L$} \Comment{EFI-GNN layers}
            \State $\textbf{X}^{(i)} = \text{matmul}(\hat{\textbf{A}}, \textbf{X}^{(i-1)})$ \Comment{node aggregation}
            \State $\textbf{X}^{(i)} = \text{matmul}(\textbf{X}^{(i)}, \textbf{W}^{(i)})$ \Comment{feature aggregation}
            \State $\textbf{X}^{(i)} = \text{mul}(\textbf{X}^{(i)}, \textbf{X}^{(1)})$ \Comment{feature crossing}
        \EndFor
        \vspace{0.3cm}
        
        \State $\textbf{X}^{(\text{out})} = \text{concat}( [ \textbf{X}^{(1)}, \textbf{X}^{(2)}, ..., \textbf{X}^{(L)} ], \text{axis=1})$
        \State $\hat{\textbf{Y}} = \text{matmul}(\textbf{X}^{(\text{out})}, \textbf{W}^{(\text{out})})$ \Comment{prediction}
    
    \end{algorithmic}
    
    \label{alg:gnc_cross_train}

\end{algorithm}


==> figures/efi-gnn_architecture.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{resources/efi-gnn_architecture.pdf}
    \caption{The overall architecture of EFI-GNN}
    \label{fig:EFI-GNN_architecture}
\end{figure*}


==> figures/feature_interactions.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{resources/feature_interactions}
    \caption{Feature interactions via hand-crafted features}
    \label{fig:feature_interactions}
\end{figure*}


==> sections/additional_visualization.tex <==
\section{Additional Study on Visualization of Feature Interactions}

    We showed that our EFI-GNN is an interpretable AI model and visualized the feature interactions.
    We additionally visualize first-order and second-order feature interactions with different hyper-parameter settings.
    Figure \ref{fig:units}, Figure \ref{fig:layers}, and Figure \ref{fig:seeds} are the visualizations of the first-order feature interactions on the different number of units, layers, and different seeds, respectively.
    The first-order feature interactions have the same trend.
    It indicates that EFI-GNN pays attention to the same features across the different hyper-parameter settings and shows EFI-GNN is reliable.
    Figure \ref{fig:units2} is the visualization of the second-order feature interactions on the different numbers of units.
    Unlike first-order feature interactions, it is hard to find any patterns or trends in second-order feature interactions.
    We anticipate that the node aggregation in an EFI-GNN layer causes this problem.
    An EFI-GNN layer aggregates the features of neighboring nodes.
    This may make it more challenging to capture stable patterns of feature interactions.
    Our future work is to find out exactly why this problem is caused.

    \input{figures/units.tex}
    \input{figures/layers.tex}
    \input{figures/seeds.tex}
    \input{figures/units2.tex}


==> sections/hyperparameter_settings.tex <==
\section{Hyper-parameter Settings}

    We optimize the hyper-parameters of experimental models with the greedy search algorithm.
    Table \ref{tbl:hparam1} shows the hyper-parameter settings on Cora, CiteSeer, and PubMed.
    For a fair comparison, we use the same hyper-parameter setting on OGB datasets.
    Table \ref{tbl:hparam2} shows the hyper-parameter setting on OGB datasets.

    \input{tables/hyperparameter_settings_cite.tex}
    \input{tables/hyperparameter_settings_ogb.tex}


==> tables/hyperparameter_settings_ogb.tex <==
\begin{table}[h!]

    \centering
    
    \begin{tabular}{cc}
    
        \hline\hline
        
        \textbf{\# GNN Layer} & 1 \\
        \textbf{\# EFI-GNN Layer} & 1 \\
        \textbf{\# Units} & 128 \\
        \textbf{Learning Rate} & 0.01 \\
        \textbf{Weight Decay} & no \\
        \textbf{Dropout} & 0.3 \\
        \textbf{Activation} & leaky relu \\
        \textbf{Skip Conn} & no \\
        \textbf{Batch Norm} & yes \\
        
        \hline\hline
    
    \end{tabular}
    
    \caption{Hyper-parameter setting on OGB datasets}
    
    \label{tbl:hparam2}
    
\end{table}

